Two-stage and Lagrangian Dual Decision Rules for Multistage Adaptive Robust Optimization

In this work, we design primal and dual bounding methods for multistage adaptive robust optimization (MSARO) problems motivated by two decision rules rooted in the stochastic programming literature. From the primal perspective, this is achieved by applying decision rules that restrict the functional forms of only a certain subset of decision variables resulting in an approximation of MSARO as a two-stage adjustable robust optimization problem. We leverage the two-stage robust optimization literature in the solution of this approximation. From the dual perspective, decision rules are applied to the Lagrangian multipliers of a Lagrangian dual of MSARO, resulting in a two-stage stochastic optimization problem. As the quality of the resulting dual bound depends on the distribution chosen when developing the dual formulation, we define a distribution optimization problem with the aim of optimizing the obtained bound and develop solution methods tailored to the nature of the recourse variables. Our framework is general-purpose and does not require strong assumptions such as a stage-wise independent uncertainty set, and can consider integer recourse variables. Computational experiments on newsvendor, location-transportation, and capital budgeting problems show that our bounds yield considerably smaller optimality gaps compared to the existing methods.

==> Sections/literature.tex <==
\section{Literature Review}
\subsection{Scalability of \MSARO{}}
\MSARO{} \emph{can} be scalable sometimes \citep{ben1999robust, guslitser2002uncertainty, bertsimas2015tight}.

\subsection{Decision Rules for \MSARO{} (Primal)}
\subsubsection{Linear Decision Rules}
LDRs are sometimes optimal:
\begin{itemize}
	\item \emph{Optimality of affine policies in multistage robust optimization} \citep{bertsimas2010optimality}:\\
	For 1-dimensional constrained \MSARO{} problem of:
\begin{subequations}
	\begin{align}
		&\min_{u_1}\Big( c_1u_1 + \max_{w_1}\Big[h_1(x_2) + \dots + \min_{u_k} \big(c_ku_k + \max_{w_k}\big[h_k(x_{k+1}) + \dots \\
		&\qquad + \min_{u_T}(c_Tu_T  + \max_{w_T}h_T(x_{T+1})) + \dots \big] \big) \Big]\Big)\nonumber\\
		&x_{k+1} = x_k + u_k + w_k\\
		&u_k\in[L_k,U_k],
	\end{align}
\end{subequations}
where $ w_k $ is a random variable in a bounded interval, $ h_k(.) $ are extended real and convex functions, $ c_k\geq 0 $ are known and $ x_1 $ is given, LDR policies on recourse decisions $ u_k $ are optimal. So: ($ i $) 1-dimensional, ($ ii $) no first-stage decisions, ($ iii $) linear ordering costs $ c_k $, ($ iv $) uncertainty set consists of bounded intervals.
	\item \emph{On the power and limitations of affine policies in two-stage adaptive optimization} \citep{bertsimas2012power}:\\
	Let $ u^\star(w) \in\arg\min_u f(w,u) $ denote the Bellman-optimal response by the decision maker in the following problem:
	\begin{equation}\label{eq:problem}
	\max_{w\in\mathcal{W}} \min_{u(w)} f(w,u),
	\end{equation}
	where $ \mathcal{W}\subseteq \mathbb{R}^n $. If $ \mathcal{W} $ is a simplex and $ f(w,Qw+q) $ is convex in $ w $ for any $ Q\in \mathbb{R}^{m\times n}, q\in \mathbb{R}^m$, then we have
	$$\max_{w\in\mathcal{W}}f(w,u^\star(w)) =  \max_{w\in\mathcal{W}}f(w,\hat{Q}w+\hat{q}) ,$$
	for some $\hat{Q}\in \mathbb{R}^{m\times n}, \hat{q}\in \mathbb{R}^m$,  i.e., a worst-case affine optimal policy exists that matches $ u^\star(w) $ on all the points in $ \text{ext}(\mathcal{W}) $.  For comparison, the result of \cite{bertsimas2010optimality} translates to the following:
	\begin{itemize}
		\item $ \mathcal{W} = \mathcal{H}_n $ is the unit hypercube in $ \mathbb{R}^n $,
		\item $ u: \mathcal{W} \rightarrow \mathbb{R}  $,
		\item $ f(w,u) = a_0 + a^\top w + c u + g(b_0 + b^\top w + u) $, where $ a_0 + b_0, c\in\mathbb{R}, a,b\in\mathbb{R}^n $ and $ g: \mathbb{R}\rightarrow\mathbb{R} $ is any convex function. 
	\end{itemize}
	\item \emph{Supermodularity and affine policies in dynamic robust optimization} \citep{iancu2013supermodularity}:\\
	For a \eqref{eq:problem}, if the uncertainty sets are integer sublattices of the unit hypercube, the DP value functions are convex and supermodular in the uncertain parameters and a \emph{certain} technical condition is satisfied, the LDRs provide optimal policies for recourse decisions.
\end{itemize}

In all these cases, we have fixed recourse. Without fixed recourse, LDRs are NP-hard for two-stage ARO \citep{guslitser2002uncertainty,ben2004adjustable}. 

\subsection{Truncated Linear Decision Rules}
\emph{Robust approximation to multiperiod inventory management}\citep{see2010robust}

\subsection{Segregated Linear}
\begin{itemize}
	\item \emph{A linear decision-based approximation approach to stochastic programming} \citep{chen2008linear}
	\item \emph{Uncertain linear programs: Extended affinely adjustable robust counterparts} \citep{chen2009uncertain}
	\item \emph{Distributionally robust optimization and its tractable approximations} \citep{ goh2010distributionally}
\end{itemize}

\subsection{Piecewise Linear Decision Rules}
\begin{itemize}
	\item \emph{Generalized decision rule approximations for stochastic programming via liftings} \citep{georghiou2015generalized}
	\item \emph{A tractable approach for designing piecewise affine policies in two-stage adjustable robust optimization} \citep{ben2020tractable}
	\item \emph{Piecewise constant decision rules via branch-and-bound based scenario detection for integer adjustable robust optimization} \citep{romeijnders2020piecewise}
\end{itemize}
If an \MSARO{} problem has fixed recourse, then it can be shown that the adaptive decisions are piecewise linear \citep{bemporad2003min}.

\subsection{Polynomial Decision Rules}
\citep{bertsimas2011hierarchy}.\\
Approximations: \cite{parrilo2000structured} and \cite{lasserre2009convexity}.\\
Quadratic decision rules:
\begin{itemize}
	\item \emph{A hierarchy of near-optimal policies for multistage adaptive optimization} \citep{bertsimas2011hierarchy}
	\item \emph{Scenario-free stochastic programming with polynomial decision rules} \citep{bampou2011scenario}
	\item \emph{Distributionally robust multi-item newsvendor problems with multimodal demand distributions} \citep{hanasusanto2015distributionally}
\end{itemize}

\subsection{Decision Rules for \MSARO{} (Dual)}
\begin{itemize}
	\item \emph{Scenario-free stochastic programming with polynomial decision rules} \citep{bampou2011scenario}
	\item \emph{Primal and dual linear decision rules in stochastic and robust optimization} \citep{kuhn2011primal}
	\item \emph{A scenario approach for estimating the suboptimality of linear decision rules in two-stage robust optimization} \citep{hadjiyiannis2011scenario}
	\item \emph{Generalized decision rule approximations for stochastic programming via liftings} \citep{georghiou2015generalized}
	\item \emph{Duality in two-stage adaptive linear optimization: Faster computation and stronger bounds} \citep{bertsimas2016duality}
\end{itemize}

\subsection{Global Optimization of \MSARO{} (Exact Methods)}
\subsubsection{Two-stage ARO}
\noindent\textbf{Benders Decomposition}
\begin{itemize}
	\item \emph{Adaptive robust optimization for the security constrained unit commitment problem} \cite{bertsimas2012adaptive}
	\item \emph{Exploiting the structure of two-stage robust optimization models with exponential scenarios} \citep{hashemi2020exploiting}
\end{itemize}

\noindent\textbf{Column \& Constraint Generation} -
\emph{Solving two-stage robust optimization problems using a column-and-constraint generation method} \citep{zeng2013solving}

\noindent\textbf{Extreme Point Enumeration \& LDRs} -
\emph{A Primal--Dual Lifting Scheme for Two-Stage Robust Optimization} \citep{georghiou2020primal}.

\noindent\textbf{Fourier-Motzkin Elimination} -
\emph{Adjustable robust optimization via fourier--motzkin elimination} \citep{zhen2018adjustable}.

\subsubsection{Robust Dual Dynamic Programming}
Extension of Benders Decomposition to multi-stage setting \citep{georghiou2019robust}.

\subsection{Global Optimization of \MSARO{} (Approximations)}
\subsubsection{Uncertainty set partitioning}
Gives us a sequence of improving approximations:
\begin{itemize}
	\item \emph{Multistage robust mixed-integer optimization with adaptive partitions} \citep{bertsimas2016multistage}
	\item \emph{Multistage adjustable robust mixed-integer optimization via iterative splitting of the uncertainty set} \citep{postek2016multistage}
\end{itemize}
\subsubsection{Copositive Programming}
\noindent\textbf{Two-stage ARO} -
Equivalent COP formulations for ARO. Conservative semidefinite approximation for reformulations:
\begin{itemize}
	\item \emph{Conic programming reformulations of two-stage distributionally robust linear programs over wasserstein balls} \citep{hanasusanto2018conic}.
	\item \emph{A copositive approach for two-stage adjustable robust optimization with uncertain right-hand sides} \citep{xu2018copositive}.
\end{itemize}
\textbf{\MSARO{}} -
\emph{Improved decision rule approximations for multi-stage robust optimization via copositive programming} \citep{xu2018improved}.\\
Equivalent COP formulations for decision rule-restricted \MSARO:
\begin{itemize}
	\item Non-fixed recourse: LDR-restricted approximation has an exact COP reformulation of polynomial size.
	\item Quadratic DR-restricted approximation with fixed recourse has an exact COP reformulation.
\end{itemize}

\subsection{\MSARO{} with Endogenous Uncertainty}
\cite{feng2020multistage} and \cite{vayanos2020robust}.


